ANPL: Towards Natural Programming with Interactive Decomposition

Though LLMs are capable of generating plausible programs, it's challenging to interact with the LLMs further to revise the program, especially if the user's specific requirements are different from the initial proposal. In this paper, we introduce ANPL, an interactive programming system that ensures users can always refine the generated code towards their specific programmatic intents via structured decompositions. Borrowing the paradigm of sketching from program synthesis, an ANPL program consists of a set of input-outputs that it must satisfy, a ``sketch'' -- control/data flow expressed in precise code (e.g. Python), and ``holes'' -- sub-modules to be implemented by the LLM specified with natural language. The user revises an ANPL program by either modifying the sketch, changing the language used to describe the holes, or providing additional input-outputs to a particular hole, turning it into a sub-ANPL program that can be solved recursively. This workflow allows the users to offload programming burdens to the LLM as much as possible while retaining the ability to pinpoint and resolve bugs locally, without exposing the rest of the program to the LLM. We deploy ANPL on the Abstraction and Reasoning Corpus (ARC), a set of unique tasks that are challenging for state-of-the-art AI systems, showing it outperforms baseline programming systems that (a) without the ability to decompose tasks interactively and (b) without the guarantee that the modules can be correctly composed together. Additional evaluations on APPS, HumanEval, and real-world programming tasks have validated that the ANPL framework is applicable to multiple programming domains. We release the ANPL solutions to the ARC tasks as a dataset, providing insights into how humans decompose novel tasks programmatically. See our code at https://iprc-dip.github.io/ANPL/.

==> figures/pseudocode.tex <==
% \centering
% \begin{minipage}{\textwidth}
% \begin{subfigure}
% \begin{minipage}{0.44\textwidth}
% \centering
% \begin{figure*}[t]
% \vspace{-10px}
% \begin{lstlisting}[basicstyle=\fontsize{6}{8}\selectfont\ttfamily]


\begin{lstlisting}[breaklines=true,numbers=none]
def compiling(ANPL):
  while `ANPL program has a hole`(ANPL):
    hole = `return the first hole in ANPL program`(ANPL):
    generated_code = LLM(ANPL, hole.descriptions, hole.IOs)
    dependency_graph = `analyze generated code, return dependency graph with topology sort`(generated_code)
    entry_nodes = `return all entry nodes of the dependency graph with topology sort`(dependency_graph)
    if `the hole has been named by the user`(hole):
      new_dependency_graph = `remove unrelated nodes in the dependency graph`(dependency_graph, hole)
      ANPL = `fill the hole with generated code according to the dependency graph`(ANPL, generated_code, new_dependency_graph)
    elif len(entry_nodes) == 1:
      ANPL = `fill the hole with generated code according to the dependency graph`(ANPL, generated_code, dependency_graph)
    else:
      # The dependency graph has multiple entry nodes, re-generate the hole.
      continue
  return ANPL

def compilingDiff(ANPL_old, ANPL_new):
  if `ANPL program has a hole`(ANPL_new):
    ANPL_new = compile(ANPL_new)
  ANPL = `merge two dependency graphs according to the merging principle of intention: user_new > user_old > LLM_old > LLM_new`(ANPL_old, ANPL_new)
  return ANPL
\end{lstlisting}
% \vspace{-10px}
% \caption{Pseudocode in the style of Parsel describing how Parsel compiles programs and debugs programs.}
% \label{shortpseudo}
% \vspace{-10px}
% \end{figure*}
% \end{minipage}
    



\begin{minted}[
def compiling(ANPL):


\end{minted}

\begin{comment}
\begin{figure}[t]
  \centering
\begin{minted}[
frame=lines,
framesep=2mm,
baselinestretch=1.2,
bgcolor=backcolour,
fontsize=\scriptsize,
linenos=0
]{python}
def identify(input_grid):
    """
    identify the smallest repeating unit
    """

def main(input_grid: np.ndarray) -> np.ndarray:
    unit = identify(input_grid)
    output_grid = "extend the input grid to 9x3 with unit"(input_grid, unit)
    return output_grid
\end{minted}
% \vspace{-9px}
  \caption{The \xname/ compiler in the style of \xname/.}
\end{figure}
\end{comment}
